Unicorn: Reasoning about Configurable System Performance through the lens of Causality

Modern computer systems are highly configurable, with the total variability space sometimes larger than the number of atoms in the universe. Understanding and reasoning about the performance behavior of highly configurable systems, over a vast and variable space, is challenging. State-of-the-art methods for performance modeling and analyses rely on predictive machine learning models, therefore, they become (i) unreliable in unseen environments (e.g., different hardware, workloads), and (ii) may produce incorrect explanations. To tackle this, we propose a new method, called Unicorn, which (i) captures intricate interactions between configuration options across the software-hardware stack and (ii) describes how such interactions can impact performance variations via causal inference. We evaluated Unicorn on six highly configurable systems, including three on-device machine learning systems, a video encoder, a database management system, and a data analytics pipeline. The experimental results indicate that Unicorn outperforms state-of-the-art performance debugging and optimization methods in finding effective repairs for performance faults and finding configurations with near-optimal performance. Further, unlike the existing methods, the learned causal performance models reliably predict performance for new environments.

==> 11_scalability.tex <==
\section{Scalability of \tool}

To examine the scalability of \tool, we evaluate \tool using the speedtest workload of SQLite database to resolve the latency faults due to misconfigurations. SQLite database workloads have a higher number of configurable options compared to image, NLP, and speech workloads. SQLite workloads exhibit unique compute, memory, data reuse characteristics, and higher memory accesses. As a result, SQLite exposes new system design opportunities to enable efficient inference and many complex interactions between software options. We evaluate \tool on the following two scenarios:

\noindent\paragraph{Increasing number of configuration options.} In the first scenario, we perform a sensitivity analysis of \tool by increasing the size of the configuration space. We start with 47 configuration options which we manually select based on important hardware, kernel configuration options, and system events recommended in performance blogs. Then we increase the number of configuration options to 330 by including 206 \texttt{sysctl} kernel configuration options that can be tuned without rebooting the system. Finally, we extend the number of configuration options to 530 by including all the system events tracked by \textsc{iperf}. In each case, we track the time required to discover the causal structure, evaluate the counterfactual queries and resolve a latency fault.  

\noindent\paragraph{Increasing number of configuration options' values.} \tool recommends a fix by computing individual treatment effect to evaluate counterfactual queries. The number of these counterfactual queries depends on the number of values taken by a configuration option. If a configuration option can be set to a large number of values, the number of counterfactual queries needed to be evaluated also increases. To determine the behavior of \tool in such scenarios, we evaluate \tool by increasing the number of values the hardware and kernel configuration options can be set at while resolving the latency faults in the SQLite speedtest workload. 


==> 7_discuss.tex <==
\section{Threats to Validity}
\label{sect:threat}



==> 8_threats.tex <==
\section{Threats to Validity}
\label{sect:threats}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> colors.tex <==
\sethlcolor{lightgray}
\definecolor{pink}{RGB}{252,145,149}
\definecolor{lightpink}{RGB}{252,145,149}
\definecolor{lightgray}{gray}{0.8}
\definecolor{darkgray}{gray}{0.6}
\definecolor{Gray}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.85}
\definecolor{Blue}{RGB}{0,29,193}
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45} 
\definecolor{pink}{RGB}{231,95,110}
\definecolor{lightergray}{rgb}{0.85, 0.85, 0.85}
\definecolor{lightestgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{codebg}{HTML}{F4F4F4}

% ---- Grays ----
\definecolor{gray05}{gray}{0.95}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray90}{gray}{0.10}


==> figures/CAUPER_overview.tex <==
\begin{figure}[t!]
    % \setlength{\belowcaptionskip}{-3em}
    \centering
    \includegraphics*[width=\linewidth]{UnicornOverview}
    \caption{\small {Overview of \ourapproach}}
    \vspace{-2em}
    \label{fig:overview}
    % \rayb{I have questions about this figure. Let's talk in the morning}
\end{figure}

==> figures/DAG_tie_breaking.tex <==
\begin{figure}[t!]
    \centering
    \subfloat[][FCI (PAG).]{\includegraphics[width=0.3\linewidth]{fig__fci_sample_1.pdf}\label{fig:fci_samp}}
    %
    ~
    %
    \subfloat[][NOTEARS (DAG).]{\includegraphics[width=0.3\linewidth]{fig__notears_sample_1.pdf}\label{fig:notears_samp}}
    %
    ~
    %
    \subfloat[][Final ADMG.]{\includegraphics[width=0.3\linewidth]{fig__DAG_sample.pdf}\label{fig:dag_samp}}
    \caption{\small Resolving ties between FCI and NOTEARS.}
    \label{fig:ties}
\end{figure}

==> figures/cauper_samp.tex <==
\begin{figure}[t!]
    \setlength{\belowcaptionskip}{-1em}
    \centering

    % \subfloat[][Using \tool for debugging.]{
        \includegraphics[width=\linewidth]{fig__cauper_samp.pdf}\label{fig:cauper_samp}
        % }
    %
    %
    %
    % \subfloat[][Using \texttt{iperf} and \texttt{top} command line profilers for debugging.]{\includegraphics[width=0.5\linewidth]{fig__iperf.pdf}\label{fig:iperf_samp}}
    
    \caption{\small A simplified causal model used in \tool. \protect\edgeone~shows the causal paths between configurations and between configurations and non-functional properties like latency, energy consumption, \etc. The numbers represent the magnitude of causal effect.}
    % \caption{\small Mechanisms to debug non-functional faults. Here, (a) shows a simplified causal model \tool builds to debug non-functional faults, \eg, when debugging for latency, the \red{$\boldsymbol{\longrightarrow}$} shows the causal paths from the configurations to latency and the numbers represent the magnitude of causal effect; (b) shows an sample \texttt{iperf} (for network load information) and \texttt{top} (for system load information) trace used to pinpoint and fix a real-world performance bug~\cite{HighCPUu7:online}}
    \label{fig:sample}
\end{figure}

==> figures/fci_samp.tex <==
\begin{figure*}[tbp!]
    % \setlength{\belowcaptionskip}{-1em}
    \subfloat[Sample Observational Data]{
        \resizebox{0.24\linewidth}{!}{\adjustbox{valign=b}{%
        \begin{tabular}{@{}c|ccc@{}cc|r|}
            \clineB{2-7}{2}
        \multicolumn{1}{c|}{} & \multicolumn{3}{c}{\textit{(Configurable Options)}} & &  \multicolumn{1}{c|}{\textit{(Sys. Events)}} & Latency \bigstrut[t]\\
        \multicolumn{1}{c|}{} & GPU Growth &$\vdots$ &Swap Mem & &Resource Use &  \etc. \\ \hlineB{2}
        $c_1$ & $0.25$ &$\vdots$& $2~Gb$ & & $10\%$ & \cellcolor{gray05}1 sec, \dots \\
        $c_2$ & $0.5$ &$\vdots$& $1~Gb$ & & $20\%$ & \cellcolor{gray05}2 sec, \dots \\
        $c_3$ & $0.66$ &$\vdots$& $1.5~Gb$ & & $40\%$ & \cellcolor{gray05}1.5 sec, \dots \\
        $c_4$ & $0.75$ &$\vdots$& $3~Gb$ & & $60\%$ & \cellcolor{gray05}3 sec, \dots \\
        $\vdots$ & $\vdots$ & $\vdots$& $\vdots$ & \multicolumn{1}{@{}c@{}}{$\ddots$} & $\vdots$ & \multicolumn{1}{c|}{\cellcolor{gray05}$\vdots$} \\
        $c_n$ & $1.0$ &$\vdots$& $4~Gb$ & & $40\%$ & \cellcolor{gray05}0.1 sec, \dots \\ \hlineB{2}
        \end{tabular}}}
        \label{tab:fci_samp_a}}
 \qquad\subfloat[Dense Graph]{\includegraphics*[width=0.2\linewidth, valign=b]{dense_graph.pdf}\label{fig:fci_samp_b}} 
 \qquad
 \subfloat[SCM Skeleton]{\includegraphics*[width=0.28\linewidth, valign=b]{final_admg.pdf}\label{fig:fci_samp_c}}
 \qquad
 \subfloat[Partial Ancestral Graph (PAG) from FCI]{\includegraphics*[width=0.28\linewidth]{final_admg.pdf}\label{fig:fci_samp_d}}
 \vspace{-.45cm}
 \subfloat[Orienting partially directed edges from \protect\fig{fci_samp_d} using entropy]{\includegraphics*[width=0.35\linewidth, valign=b]{fig__fci_entropy_flow.pdf}\label{fig:fci_samp_e}}
\qquad
 \subfloat[Final ADMG]{\includegraphics*[width=0.28\linewidth, valign=b]{final_admg.pdf}\label{fig:fci_samp_f}}
% %  
\caption{\small {From observational data to a fully connected graph, a skeleton graph, and finally an acyclic directed mixed graph (ADMG).}}

% \rayb{Parts of figure e is not clear. Let's talk in the morning. }
\label{tab:fci_example}\end{figure*}



==> figures/objectives_overlap.tex <==
\begin{wrapfigure}[11]{R}{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig__venn.pdf}
    \caption{\small Summary of \protect\tab{perf_faults_summary}. Numbers in {\color[HTML]{CC3333} \bfseries red} indicate cases with more than one non-functional faults.}
    \label{fig:objectives_overlap}
\end{wrapfigure}

==> figures/software_stack.tex <==

\begin{figure}[t]
    \setlength{\belowcaptionskip}{-1.25em}
    \centering
    \includegraphics[width=\linewidth]{fig__intro_a.pdf}
    \caption{Observational data (in Fig.~\protect\ref{fig:intro_fig}a)  (incorrectly) shows that high \gpugrowth leads to high latency. The trend is reversed when the data is segregated by \swapmem.}
    \label{fig:intro_fig}
\end{figure}

% \begin{figure}[tp!]
%     \setlength{\belowcaptionskip}{-0.8em}
%     \centering
%     \subfloat[\gpugrowth v. Latency]
%     {\label{fig:intro_a}\includegraphics[width=0.45\linewidth]{fig__intro_1.pdf}}~
%     \subfloat[Observations segregated on \swapmem]
%     {\label{fig:intro_b}\includegraphics[width=0.45\linewidth]{fig__intro_2.pdf}}
%     \\[0.05em]
%     % \subfloat[Performance curves][Performance (Latency) curves]
%     % {\label{fig:intro_b}\includegraphics[width=0.68\linewidth]{fig__intro_b.pdf}}
%     \subfloat[][Causal Model]
%     {\label{fig:intro_c}\includegraphics[width=0.3\linewidth]{fig__intro_c.pdf}}\\[-1em]
%     \caption{\smallObservational data can sometimes lead to misleading inference. In \protectFig.~\ref{fig:intro_fig}a, the data (incorrectly) shows that high \gpugrowth leads to high latency. In \protectFig.~\ref{fig:intro_fig}b, the trend is reversed when the same data is segregated by \swapmem.}
%     \label{fig:intro_fig}
% \end{figure}


==> listings/listing__cauper.tex <==
\begin{figure}[t!]
    
    \begin{minipage}{\linewidth}
            \algcauper
        %     \caption{\small \tool framework.}
        \end{minipage}
        \\[-1em]
    %     \begin{minipage}{\linewidth}
    %             \algquery
    %             % \caption{\small Generating interventions.}
    % \end{minipage}
\end{figure}

% \begin{figure*}
%     \subfloat[][\tool]{
%         \begin{minipage}{0.5\linewidth}
%             \algcauper
%         \end{minipage}}
%     \subfloat[][Counterfactual query generation]{
%         \begin{minipage}{0.5\linewidth}
%             \algquery
%         \end{minipage}}
% \end{figure*}

==> spacing.tex <==
% \setlength{\belowcaptionskip}{-10pt}
% \setlength{\floatsep}{10pt}
% \setlength{\textfloatsep}{10pt}
% \setlength{\dbltextfloatsep}{10pt}
% \setlength{\fboxsep}{.2pt}
\begin{comment}
% % \setlength{\multicolsep}{2.0pt}% 50% of original values


% % \DeclarePairedDelimiter\abs{\lvert}{\rvert}%
% ----- Change the spacing before and after equations globally -----
\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{2pt}
  \setlength\belowdisplayskip{2pt}
  \setlength\abovedisplayshortskip{2pt}
  \setlength\belowdisplayshortskip{2pt}
}
\makeatother

% % \makeatletter
% % \def\thm@space@setup{%
% %   \thm@preskip=0cm plus 0cm minus 0cm
% %   \thm@postskip=\thm@preskip % or whatever, if you don't want them to be equal
% % }
% % \makeatother

% % \newtheorem{definition}{Definition}

\titleformat{\subsubsection*}[runin]{\bf\normalsize}{\thesubsubsection*}{0em}{}[\xspace\mbox{}]
\titlespacing*{\subsubsection*}{0pt}{0ex plus 0ex minus 0ex}{0pt}

% % \titlespacing*{\section}{5pt}{0.3\baselineskip}{0.3\baselineskip}
% % \titlespacing*{\subsection}{3pt}{0.5\baselineskip}{0.5\baselineskip}
\titleformat*{\subsubsection}{\em\xspace}
% % \titlespacing*{\subsubsection}{2pt}{0.1\baselineskip}{0.1\baselineskip}
\end{comment}

%\titleformat{\subsubsection*}[runin]{\bf\normalsize}{\thesubsubsection*}{0em}{}[\xspace\mbox{}]
% \titlespacing*{\subsubsection*}{0pt}{0ex plus 0ex minus 0ex}{0pt}
% \setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*}%, wide=0pt}
% \setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=*}%, wide=0pt}
% \titlespacing*{\subsection}{3pt}{0.75\baselineskip}{0.75\baselineskip}


==> tables/config_options.tex <==
% \begin{table*}[h]
% \caption{\small Configurations options by each layer.}
% \small 
% \resizebox{\linewidth}{!}{\begin{tabular}[t]{p{0.35\linewidth}|p{0.3\linewidth}p{0.2\linewidth}p{0.2\linewidth}p{0.2\linewidth}}
 
% \centering
% Configuration options& & Layer&\\
% \midrule
% \multicolumn{5}{c}{Workload}\\
% \cmidrule(lr){1-5}\\ 
% &\multicolumn{4}{c}{DNN}\\
% \cmidrule(lr){2-5}\\
% Memory growth & 0, 0.1, 0.5&\\
% Logical devices & 10, 50\\ 
% \cmidrule(lr){2-5}\\
% &\multicolumn{4}{c}{SQLite}\\
% \cmidrule(lr){2-5}\\
% Cache size & 0, 0.1, 0.5&\\
% Buffer size & 10, 50\\ 
% Synchronous & 0, 1 \\
% Journal mode & Memory, Disk \\
% Temporary store & Memory, Disk \\

% \cmidrule(lr){2-5}\\
% &\multicolumn{4}{c}{x264}\\
% \cmidrule(lr){2-5}\\
% CRF & 0, 0.1, 0.5&\\
% Preset & 10, 50\\
% Bit rate & 10,100\\
% Latency & 1,2 \\
% \hline 
% \multicolumn{5}{c}{OS/Kernel}\\
% \cmidrule{1-5}\\
% Scheduler policy& CFP, NOOP\\
% Swappiness&10, 60, 100\\
% Dirty background ratio&10, 80\\
% Dirty ratio& 5, 50\\
% Sched child runs first & 0, 1 \\
% Drop caches & 0, 1, 2, 3\\
% Cache pressure & 1, 100, 500 \\

% \hline
% \multicolumn{5}{c}{Hardware}\\
% \cmidrule{1-5}\\
% & \multicolumn{1}{l}{\nano}&\multicolumn{1}{l}{\txone} & \multicolumn{1}{l}{\txtwo} & \multicolumn{1}{l}{\xavier}\\
% \cmidrule{2-2}\cmidrule{3-3}\cmidrule{4-4}\cmidrule{5-5}\\
% Active CPUs&1 - 4&1 - 4&1 - 4&1 - 4\\
% CPU freq. (GHz)&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\
% GPU freq. (GHz)& 0.1 - 1.3&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\
% EMC freq. (GHz)&0.1 - 1.8&0.3 - 2.0&0.3 - 2.0&0.3 - 2.0\\

% \bottomrule
% \end{tabular}}
% \label{tab:configurations}
% \end{table*}%}

==> tables/dag_edge_types.tex <==
% \begin{table}[tbp!]
%     \caption{\small How FCI transforms a fully connected dense graph $(G)$ to a skeleton graph $(S)$ and to Partial DAG (PAG). %Note, the nodes Y and Z are \textit{not} independent when they are not conditioned on other variables (denoted by $\dagger$); but when conditioned on X, they become independent (denoted by $\ddagger$), thus the edge $Y\text{---}Z$ is removed in the skeleton. 
%     }
%     \label{tab:fci_example}
%     \resizebox*{\linewidth}{!}{
%     \begin{tabular}{crcc}
%         \hlineB{2}
%     Dense G           & Independence & Skeleton $(S)$   & Partial DAG $(PAG)$      \bigstrut\\\hlineB{2}

%     \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_full.pdf}}} 
%     & $X\notindependent Y$     & \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_pruned.pdf}}} & \multirow{7}{*}{\raisebox{-1.25\totalheight}{\includegraphics*[width=0.2\linewidth]{fig__fci_und_dir.pdf}}} \bigstrut\\
%                       & $X\notindependent Z$     &         &          \bigstrut\\
%                       & $X\independent W$     &         &          \bigstrut\\
%                       & $Y\notindependent Z^{\dagger}$     &     &              \bigstrut\\
%                       & $Y\notindependent W$     &               &    \bigstrut\\
%                       & $Z\notindependent W$     &              &     \bigstrut\\
%                       & $Y\independent Z~|~X^{\ddagger}$   &  & \\\hlineB{2}               
%     \end{tabular}}
% \end{table}
    

    

==> tables/manual_study.tex <==
% \begin{figure}[t!]
%     \setlength{\belowcaptionskip}{-1em}
%     \centering
%     \subfloat[t][]{    
%     \resizebox{0.45\linewidth}{!}{\adjustbox{valign=b}{%
%     \begin{tabular}{lrrrr}
%         \hlineB{2}
%         Type& \rotatebox{90}{\txone~} & \rotatebox{90}{\txtwo} & \rotatebox{90}{\xavier~} & \rotatebox{90}{Total}\bigstrut\\\hlineB{2}
%         Latency & 6 & 9 & {5} & \cellcolor{gray05}20 \bigstrut[t]\\
%         Energy & 6 & 4 & {8} & \cellcolor{gray05}17 \\
%         Thermal & 5 & 2 & {2} & \cellcolor{gray05}9 \bigstrut[b]\\
%         \rowcolor{gray05} Total & 17 & 15 & 15 & \cellcolor{gray12} 47 \bigstrut\\ \hlineB{2}
%     \end{tabular}%
%     \label{tab:perf_faults_count}
%     }
%     }
%     }~
%     \subfloat[t][]{
%         \includegraphics[width=0.45\linewidth, valign=b]{fig__venn.pdf}
%         \label{fig:perf_faults_venn}
%     }    
% \caption{\small non-functional faults in reported in NVIDIA Jetson\textsuperscript (gathered from NVIDIA developer forum). (a) Distribution across hardware, (b) Distribution across fault type ({\color[HTML]{CC3333} \bfseries red} indicate cases with multiple non-functional fault types).}
% \label{tab:perf_faults_summary}
% \end{figure}

==> tables/rq1_gain.tex <==
\begin{table}[t!]
    \centering
    \caption{\small (RQ1) Performance gain (\eq{gain}) up on applying repairs prescribed by respective approaches. Larger gains (in \colorbox[HTML]{C9E7BF}{green}) are considered better. \tool achieves better $\Delta_{gain}$ overall.}
    \label{tab:rq1_2}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ll|lll|lll|lll|}
     &  & \multicolumn{3}{c|}{TX1} & \multicolumn{3}{c|}{TX2} & \multicolumn{3}{c|}{\xavier} \bigstrut\\ \clineB{3-11}{2} 
     & Software & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} & \rotatebox{90}{\tool} & \rotatebox{90}{CBI~\cite{song2014statistical}~} & \rotatebox{90}{Default~} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Latency}} & DNN Image & \cellcolor[HTML]{C9E7BF}78 & 75 & 71 & \cellcolor[HTML]{C9E7BF}75 & 53 & 46 & \cellcolor[HTML]{C9E7BF}89 & \cellcolor[HTML]{C9E7BF}89 & 61 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}86 & 70 & 60 & \cellcolor[HTML]{C9E7BF}79 & 51 & 34 & \cellcolor[HTML]{C9E7BF}89 & 67 & 80 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}76 & 72 & 66 & \cellcolor[HTML]{C9E7BF}94 & 76 & 54 & \cellcolor[HTML]{C9E7BF}90 & 77 & 64 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}29 & 27 & 10 & \cellcolor[HTML]{C9E7BF}28 & 13 & 5 & \cellcolor[HTML]{C9E7BF}35 & \cellcolor[HTML]{C9E7BF}35 & 20 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}32 & 20 & 10 & \cellcolor[HTML]{C9E7BF}32 & 10 & 11 & \cellcolor[HTML]{C9E7BF}29 & 11 & 13 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Energy}} & DNN Image & \cellcolor[HTML]{C9E7BF}77 & 41 & 18 & \cellcolor[HTML]{C9E7BF}89 & 51 & 30 & \cellcolor[HTML]{C9E7BF}79 & 53 & 41 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}76 & 51 & 9 & 67 & \cellcolor[HTML]{C9E7BF}77 & 40 & \cellcolor[HTML]{C9E7BF}69 & 47 & 30 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}71 & 42 & 19 & \cellcolor[HTML]{C9E7BF}76 & 66 & 42 & \cellcolor[HTML]{C9E7BF}76 & 47 & 35 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}32 & 16 & 9 & \cellcolor[HTML]{C9E7BF}24 & 13 & 6 & \cellcolor[HTML]{C9E7BF}32 & 20 & 5 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}25 & 13 & 12 & \cellcolor[HTML]{C9E7BF}23 & 10 & 7 & \cellcolor[HTML]{C9E7BF}26 & 19 & 6 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{Thermals}} & DNN Image & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 3 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 3 & \cellcolor[HTML]{C9E7BF}8 & 1 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN Speech & \cellcolor[HTML]{C9E7BF}4 & 3 & 3 & \cellcolor[HTML]{C9E7BF}7 & 5 & 2 & \cellcolor[HTML]{C9E7BF}3 & 2 & 3 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}7 & 3 & 4 & \cellcolor[HTML]{C9E7BF}7 & 4 & 2 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}8 & 2 & 1 & \cellcolor[HTML]{C9E7BF}5 & \cellcolor[HTML]{C9E7BF}5 & 1 & \cellcolor[HTML]{C9E7BF}8 & 3 & 2 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}6 & 5 & 2 & \cellcolor[HTML]{C9E7BF}5 & 3 & 2 & \cellcolor[HTML]{C9E7BF}3 & 1 & 1 \bigstrut\\ \hlineB{2}
    \end{tabular}%
    }
    \end{table}

==> tables/rq2.tex <==
%  \begin{table}[]
%      \centering
%      \caption{\small (RQ2) Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults. Cells highlighted in \colorbox{blue!10}{green} indicate better performance and \colorbox[HTML]{FFCCC9}{red} indicate cases where the performance drops. Note: the results are reported for two kinds of faults in TX2: (1) faults in both latency and energy; and (2) faults in latency, energy, and heat dissipation.}
%      \label{tab:rq2}
%      \resizebox{\linewidth}{!}{
%      \begin{tabular}{ll|rr|rr|rr|}
%       &  & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \multicolumn{1}{r|}{\rotatebox{90}{Default}} \bigstrut\\ \cline{3-8} 
%       & Software & \multicolumn{2}{r|}{Accuracy} & \multicolumn{2}{r|}{Recall} & \multicolumn{2}{r|}{Precision} \bigstrut\\ \hlineB{2}
%      \multicolumn{1}{l|}{\multirow{6.5}{*}{Latency and Energy}} & DNN Image & \cellcolor{blue!10}59 & 51 & \cellcolor{blue!10}44 & 35 & \cellcolor{blue!10}65 & 56 \bigstrut\\
%      \multicolumn{1}{l|}{} & DNN   Speech & \cellcolor{blue!10}66 & 49 & \cellcolor{blue!10}51 & 43 & \cellcolor{blue!10}74 & 64 \bigstrut\\
%      \multicolumn{1}{l|}{} & DNN NLP & \cellcolor{blue!10}56 & 53 & \cellcolor{blue!10}42 & \cellcolor{blue!10}42 & \cellcolor{blue!10}66 & 61 \bigstrut\\
%      \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}51 & 48 & \cellcolor{blue!10}55 & 33 & \cellcolor{blue!10}64 & 56 \bigstrut\\
%      \multicolumn{1}{l|}{} & SQLite & \cellcolor{blue!10}60 & 51 & \cellcolor{blue!10}57 & 37 & \cellcolor{blue!10}72 & 57 \bigstrut\\ \hlineB{2}
%      \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \cellcolor{blue!10}67 & 59 & \cellcolor{blue!10}69 & 60 & \cellcolor{blue!10}64 & 60 \bigstrut\\
%      \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}68 & 62 & \cellcolor{blue!10}79 & 56 & \cellcolor{blue!10}68 & 58 \bigstrut\\
%      \multicolumn{1}{l|}{} & SQLite & \cellcolor{blue!10}79 & 63 & \cellcolor{blue!10}70 & 57 & \cellcolor{blue!10}84 & 63 \bigstrut\\ \hlineB{2}\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}\bigstrut\\[-0.4cm]\hlineB{2}
%      \multicolumn{1}{l}{\multirow{9.5}{*}{Latency and Energy}} & \multicolumn{1}{r|}{$\Delta_{gain}\longrightarrow$} & \multicolumn{2}{c|}{{Latency}} & \multicolumn{2}{c|}{{Energy}} & \multicolumn{2}{c|}{{Thermals}} \bigstrut\\ \hlineB{2} 
    
%      \multicolumn{1}{l|}{} & DNN Image & \cellcolor{blue!10}52 & \multicolumn{1}{l|}{33} & \multicolumn{1}{l}{\cellcolor{blue!10}37} & \multicolumn{1}{l|}{22} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & DNN   Speech & \multicolumn{1}{l}{\cellcolor{blue!10}60} & \multicolumn{1}{l|}{25} & \multicolumn{1}{l}{\cellcolor{blue!10}54} & \multicolumn{1}{l|}{17} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & DNN NLP & \multicolumn{1}{l}{\cellcolor{blue!10}49} & \multicolumn{1}{l|}{30} & \multicolumn{1}{l}{\cellcolor{blue!10}51} & \multicolumn{1}{l|}{17} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{0} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & x264 & \multicolumn{1}{l}{\cellcolor{blue!10}23} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{\cellcolor{blue!10}12} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-2} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & SQLite & \multicolumn{1}{l}{\cellcolor{blue!10}9} & \multicolumn{1}{l|}{6} & \multicolumn{1}{l}{\cellcolor{blue!10}11} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{0} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\ \hlineB{2}
    
%      \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \multicolumn{1}{l}{\cellcolor{blue!10}54} & \multicolumn{1}{l|}{29} & \multicolumn{1}{l}{\cellcolor{blue!10}31} & \multicolumn{1}{l|}{16} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{1} \bigstrut\\
    
%      \multicolumn{1}{l|}{} & x264 & \multicolumn{1}{l}{\cellcolor{blue!10}18} & \multicolumn{1}{l|}{1} & \multicolumn{1}{l}{\cellcolor{blue!10}10} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}-1} \bigstrut\\
   
%      \multicolumn{1}{l|}{} & SQLite & \multicolumn{1}{l}{\cellcolor{blue!10}6} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l}{\cellcolor{blue!10}7} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l}{1} & \multicolumn{1}{l|}{0} \bigstrut\\ \hlineB{2}
%      \end{tabular}
%      }
%      \end{table}

\begin{table*}[]
    \centering
    \caption{\small {Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults: \textit{Energy, Latency}; and \textit{Energy, Latency, Heat}. Cells highlighted in \colorbox{blue!10}{green} indicate improvement over faults and \colorbox[HTML]{FFCCC9}{red} indicate deterioration. \tool achieves better performance overall and is much faster. Note: the results are reported for NVIDIA Jetson TX2.}}
    \label{tab:rq2}
    \footnotesize
    \resizebox{\textwidth}{!}{
        \begin{tabular}{@{}l@{}ll|llll|llll|llll|llll|llll|llll|ll|}
            \clineB{4-29}{2}
            &  &  & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{Precision} & \multicolumn{4}{c|}{Recall} & \multicolumn{4}{c|}{Gain (Latency)} & \multicolumn{4}{c|}{Gain (Energy)} & \multicolumn{4}{c|}{Gain (Heat)} & \multicolumn{2}{c|}{Time$^\dagger$} \bigstrut\\ \clineB{4-29}{2}
            % &  &  &  &  &  &  &  &  & \\[-1em]\clineB{4-29}{2} 
            
            &  &  & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{\cbi} & \rotatebox{90}{\encore} & \rotatebox{90}{\bugdoc} & \rotatebox{90}{\bfseries\tool~} & \rotatebox{90}{Others} \\ \clineB{4-29}{2}
            
            \multicolumn{1}{l}{}&\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\[-0.9em]\hlineB{2}

            & \multicolumn{1}{l|}{} & Image & \cellcolor{blue!10}\textbf{77} & 54 & 55 & 65 & \cellcolor{blue!10}\textbf{73} & 53 & 54 & 62 & \cellcolor{blue!10}\textbf{80} & 59 & 59 & 62 & \cellcolor{blue!10}\textbf{83} & 53 & 61 & 65 & \cellcolor{blue!10}\textbf{70} & 38 & 46 & 44 & \cellcolor{blue!10}\textbf{3} & 0 & 0 & 0 & \cellcolor{blue!10}\textbf{0.6} & 4 \\
            & \multicolumn{1}{l|}{} & NLP & \cellcolor{blue!10}\textbf{70} & 51 & 56 & 65 & \cellcolor{blue!10}\textbf{71} & 42 & 56 & 63 & \cellcolor{blue!10}\textbf{66} & 59 & 62 & 65 & \cellcolor{blue!10}\textbf{68} & 53 & 59 & 61 & \cellcolor{blue!10}\textbf{60} & 41 & 27 & 48 & \cellcolor{blue!10}\textbf{5} & 0 & 0 & 1 & \cellcolor{blue!10}\textbf{0.2} & 4 \\
            & \multicolumn{1}{l|}{} & Speech & \cellcolor{blue!10}\textbf{74} & 50 & 61 & 65 & \cellcolor{blue!10}\textbf{68} & 44 & 53 & 62 & \cellcolor{blue!10}\textbf{79} & 51 & 59 & 64 & \cellcolor{blue!10}\textbf{82} & 55 & 55 & 62 & \cellcolor{blue!10}\textbf{66} & 43 & 43 & 41 & \cellcolor{blue!10}\textbf{4} & \cellcolor[HTML]{FFCCC9}-2 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.7} & 4 \\
            & \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}\textbf{83} & 54 & 55 & 66 & \cellcolor{blue!10}\textbf{81} & 50 & 54 & 57 & \cellcolor{blue!10}\textbf{77} & 63 & 62 & 61 & \cellcolor{blue!10}\textbf{15} & 2 & 4 & 6 & \cellcolor{blue!10}\textbf{13} & 4 & 6 & 4 & \cellcolor{blue!10}\textbf{2} & \cellcolor[HTML]{FFCCC9}-3 & \cellcolor[HTML]{FFCCC9}-1 & 0 & \cellcolor{blue!10}\textbf{1.2} & 4 \\
           \multirow{-5}{*}{\rotatebox{90}{Energy +}} & \multicolumn{1}{l|}{\multirow{-5}{*}{\rotatebox{90}{Latency}}} & SQLite & \cellcolor{blue!10}\textbf{84} & 51 & 58 & 68 & \cellcolor{blue!10}\textbf{80} & 43 & 55 & 62 & \cellcolor{blue!10}\textbf{84} & 57 & 63 & 65 & \cellcolor{blue!10}\textbf{11} & 5 & 4 & 5 & \cellcolor{blue!10}\textbf{14} & 3 & 8 & 8 & \cellcolor{blue!10}\textbf{2} & \cellcolor[HTML]{FFCCC9}-2 & 0 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.5} & 4 \\ \hlineB{2}

           \multicolumn{1}{l}{}&\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\[-0.95em]\hlineB{2}

            & \multicolumn{1}{l|}{} & Image & \cellcolor{blue!10}\textbf{76} & 57 & 48 & 66 & \cellcolor{blue!10}\textbf{68} & 61 & 57 & 61 & \cellcolor{blue!10}\textbf{81} & 53 & 46 & 70 & \cellcolor{blue!10}\textbf{62} & 33 & 30 & 42 & \cellcolor{blue!10}\textbf{52} & 23 & 18 & 24 & \cellcolor{blue!10}\textbf{4} & 1 & 0 & 0 & \cellcolor{blue!10}\textbf{0.1} & 4 \\
            & \multicolumn{1}{l|}{} & x264 & \cellcolor{blue!10}\textbf{80} & 59 & 47 & 54 & \cellcolor{blue!10}\textbf{76} & 61 & 56 & 63 & \cellcolor{blue!10}\textbf{81} & 56 & 46 & 51 & \cellcolor{blue!10}\textbf{12} & 2 & 1 & 2 & \cellcolor{blue!10}\textbf{15} & 4 & 2 & 4 & \cellcolor{blue!10}\textbf{4} & 1 & 0 & 1 & \cellcolor{blue!10}\textbf{0.1} & 4 \\
           \multirow{-3}{*}{\rotatebox{90}{All}} & \multicolumn{1}{l|}{\multirow{-3}{*}{\rotatebox{90}{Three}}} & SQLite & \cellcolor{blue!10}\textbf{73} & 56 & 51 & 53 & \cellcolor{blue!10}\textbf{68} & 59 & 56 & 60 & \cellcolor{blue!10}\textbf{78} & 54 & 45 & 51 & \cellcolor{blue!10}\textbf{12} & 1 & 1 & 4 & \cellcolor{blue!10}\textbf{8} & 4 & 2 & 5 & \cellcolor{blue!10}\textbf{1} & 1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor[HTML]{FFCCC9}-1 & \cellcolor{blue!10}\textbf{0.1} & 4 \\ \hlineB{2}
           \multicolumn{10}{l}{$^\dagger$ Wallclock time in hours}\bigstrut
           \end{tabular}
    }
\end{table*}
    

==> tables/rq3.tex <==
\begin{table}[]
    \caption{\small (RQ3) Transferring causal models across hardware platforms. Default uses the configurations from NIVIDA's Jetpack SDK. Update 10\% uses 10\% of the available budget to sample observations from the target environment to update the causal model. Remodel uses 100\% of the allocated budget to generate new samples and build a causal model from scratch on the target hardware.}
    \label{tab:rq3}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll|rrr|rrr|rrr|rrr}
        \hlineB{2}
        \multicolumn{14}{c}{TX1 (source) $\longrightarrow$ TX2 (target)} \bigstrut\\ \hlineB{2}

        & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Accuracy} & \multicolumn{3}{c|}{Recall} & \multicolumn{3}{c|}{Precision} & \multicolumn{3}{c}{$\Delta_{gain}$} 
        
        \bigstrut\\ \clineB{3-14}{2} 
        
        &  Software & \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~} & \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}& \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}& \rotatebox{90}{Default} & \multicolumn{1}{r}{\rotatebox{90}{Update {\scriptsize 10\%~}}} & \rotatebox{90}{Remodel~}\bigstrut\\ \hlineB{2}       

    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Latency}}} & Image & 52 & 78 & 88 & 70 & 79 & 86 & 46 & 78 & 91 & 46 & 66 & 74 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 55 & 67 & 76 & 57 & 79 & 75 & 45 & 57 & 81 & 33 & 65 & 79 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 45 & 59 & 64 & 56 & 79 & 62 & 49 & 56 & 74 & 54 & 82 & 94 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 47 & 75 & 83 & 70 & 79 & 82 & 58 & 67 & 85 & 5 & 19 & 28 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 59 & 68 & 80 & 68 & 76 & 78 & 52 & 64 & 84 & 10 & 22 & 31 \bigstrut\\ \hlineB{2}
    \multicolumn{14}{c}{TX2 (source) $\longrightarrow$ XAVIER (target)} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Energy}}} & Image & 53 & 70 & 84 & 48 & 71 & 86 & 51 & 59 & 78 & 30 & 81 & 88 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 50 & 71 & 77 & 53 & 75 & 80 & 49 & 68 & 74 & 40 & 59 & 67 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 57 & 66 & 73 & 45 & 74 & 70 & 43 & 53 & 77 & 42 & 69 & 76 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 54 & 70 & 79 & 46 & 79 & 77 & 42 & 65 & 83 & 6 & 13 & 24 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 45 & 65 & 82 & 48 & 79 & 70 & 47 & 63 & 81 & 7 & 16 & 23 \bigstrut\\ \hlineB{2}
    \multicolumn{14}{c}{Xavier (source) $\longrightarrow$ TX1 (target)} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox{90}{Thermals}}} & Image & 53 & 62 & 65 & 69 & 61 & 80 & 58 & 64 & 64 & 3 & 4 & 4 \bigstrut\\
    \multicolumn{1}{l|}{} & Speech & 55 & 60 & 69 & 69 & 59 & 76 & 52 & 63 & 69 & 3 & 3 & 4 \bigstrut\\
    \multicolumn{1}{l|}{} & NLP & 57 & 58 & 66 & 69 & 63 & 81 & 53 & 63 & 63 & 3 & 5 & 7 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & 51 & 58 & 68 & 73 & 51 & 76 & 54 & 71 & 66 & 1 & 4 & 7 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & 54 & 58 & 70 & 70 & 62 & 75 & 48 & 66 & 66 & 1 & 6 & 6 \bigstrut\\ \hlineB{2}
    \end{tabular}
    }
    \end{table}

==> tables/study_systems.tex <==
% \begin{table}[t!]
%     \caption{\small Overview of workloads used in our experiments.}
%     \label{tab:perf_faults_summary}
%     \centering
%     \resizebox{0.9\linewidth}{!}{%
%     \begin{tabular}{lrrrr}
%     \hlineB{2}
%     Workload & Domain & $d$ & $|C|$ & $|H|$\\\hlineB{2}
%     Xception & Image recognition (DNN) & 13 & 1408 & 4 \\
%     BERT & Natural language processing (DNN) & 13 & 1376 & 4 \\
%     DeepSpeech & Speech recognition (DNN) & 13 & 1128 & 4 \\
%     SQLite & Database & 17 & 1684 & 3 \\
%     x264& Video encoding & 19 & 1843 & 3 \\ 
    
%     \end{tabular}%
% }
% \end{table}

\begin{table}[]
    \centering
    \caption{\small (RQ2) Efficiency of \tool in detecting and repairing the root-cause of multiple non-functional faults. Cells highlighted in \colorbox[HTML]{C9E7BF}{green} indicate better performance and \colorbox[HTML]{FFCCC9}{red} indicate cases where the performance drops. Note: the results are reported for two kinds of faults in TX2: (1) faults in both latency and energy; and (2) faults in latency, energy, and heat dissipation.}
    \label{tab:rq2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|r|rrrrr|}
     &  & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \rotatebox{90}{Default} & \multicolumn{1}{r|}{\rotatebox{90}{\tool}} & \multicolumn{1}{r|}{\rotatebox{90}{Default}} \bigstrut\\ \cline{3-8} 
     & Software & \multicolumn{2}{r|}{Accuracy} & \multicolumn{2}{r|}{Recall} & \multicolumn{2}{r|}{Precision} \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{6.5}{*}{Latency and Energy}} & DNN Image & \cellcolor[HTML]{C9E7BF}59 & 51 & \cellcolor[HTML]{C9E7BF}44 & 35 & \cellcolor[HTML]{C9E7BF}65 & 56 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN   Speech & \cellcolor[HTML]{C9E7BF}66 & 49 & \cellcolor[HTML]{C9E7BF}51 & 43 & \cellcolor[HTML]{C9E7BF}74 & 64 \bigstrut\\
    \multicolumn{1}{l|}{} & DNN NLP & \cellcolor[HTML]{C9E7BF}56 & 53 & \cellcolor[HTML]{C9E7BF}42 & \cellcolor[HTML]{C9E7BF}42 & \cellcolor[HTML]{C9E7BF}66 & 61 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}51 & 48 & \cellcolor[HTML]{C9E7BF}55 & 33 & \cellcolor[HTML]{C9E7BF}64 & 56 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}60 & 51 & \cellcolor[HTML]{C9E7BF}57 & 37 & \cellcolor[HTML]{C9E7BF}72 & 57 \bigstrut\\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{3}{*}{All three}} & DNN Image & \cellcolor[HTML]{C9E7BF}67 & 59 & \cellcolor[HTML]{C9E7BF}69 & 60 & \cellcolor[HTML]{C9E7BF}64 & 60 \bigstrut\\
    \multicolumn{1}{l|}{} & x264 & \cellcolor[HTML]{C9E7BF}68 & 62 & \cellcolor[HTML]{C9E7BF}79 & 56 & \cellcolor[HTML]{C9E7BF}68 & 58 \bigstrut\\
    \multicolumn{1}{l|}{} & SQLite & \cellcolor[HTML]{C9E7BF}79 & 63 & \cellcolor[HTML]{C9E7BF}70 & 57 & \cellcolor[HTML]{C9E7BF}84 & 63 \bigstrut\\ \hlineB{2}\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{l}{}\bigstrut\\[-0.4cm]\hlineB{2}
    \multicolumn{1}{l}{\multirow{9.5}{*}{Latency and Energy}} & \multicolumn{1}{r|}{$\Delta_{gain}\longrightarrow$} & \multicolumn{2}{c|}{{Latency}} & \multicolumn{2}{c|}{{Energy}} & \multicolumn{2}{c|}{{Thermals}} \bigstrut\\ \hlineB{2} 
    
    \end{tabular}
    }
    \end{table}


==> tables/systems.tex <==
\begin{table}
 \caption{\small Summary of hardware systems, software systems, and configuration options. Note: Some configuration options do not apply to certain software systems (we highlight these with $\cdot$). We also include 17 non-intervenable systems events.}
 \label{tab:systems}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}ll|ccc|@{}c|c@{}}
        \hlineB{2}
       

        & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Deep Neural Network} & \multicolumn{1}{c|}{Database} & \multicolumn{1}{c}{Encoder}
        
        \\ \clineB{3-7}{1.5}
        
        &  Config Options &{\rotatebox[origin=c]{0}{Image}~\textsuperscript{\red{a}}} & {\rotatebox[origin=c]{0}{NLP}}~\textsuperscript{\red{b}} & {\rotatebox[origin=c]{0}{Speech}}~\textsuperscript{\red{c}} & SQLite &x264  \\ \hlineB{2}       

    \multicolumn{1}{l|}{\multirow{4}{-1em}{\rotatebox{90}{Hardware}}} & Cpu cores  & {\footnotesize\color{gray50} $\checkmark$} & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}  \\
    \multicolumn{1}{l|}{} & EMC freq      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}     \\
    \multicolumn{1}{l|}{} & CPU freq                                      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & GPU freq                                    & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}     \\ \hlineB{2}
   
    \multicolumn{1}{l|}{\multirow{8}{*}{\rotatebox{90}{OS/Kernel}}} & Scheduler policy                                     & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Sched child runs first                                  & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Sched rt runtime                     & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$} \\
    \multicolumn{1}{l|}{} & Drop caches                                           & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}   \\
    \multicolumn{1}{l|}{} & Dirty background ratio                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}         & {\footnotesize\color{gray50} $\checkmark$}   \\ 
     \multicolumn{1}{l|}{} & Dirty ratio                                         & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}  \\
          \multicolumn{1}{l|}{}&VFS cache pressure                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}                      \\
      \multicolumn{1}{l|}{}&Swappiness                                      & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\checkmark$}  \\ \hlineB{2}
    \multicolumn{1}{l|}{\multirow{9}{*}{\rotatebox{90}{Application}}} & GPU Memory growth                               & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {$\cdot$} & {$\cdot$} \\
    
    \multicolumn{1}{l|}{} & Clear session                & {\footnotesize\color{gray50} $\checkmark$}                                 & {\footnotesize\color{gray50} $\checkmark$}    & {\footnotesize\color{gray50} $\checkmark$}   & {$\cdot$} & {$\cdot$} \\
               
     \multicolumn{1}{l|}{}& Preset                       & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}                   \\ 
    \multicolumn{1}{l|}{} & Filter& {\footnotesize\color{gray50} $\cdot$}             & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}\\ 
    
     \multicolumn{1}{l|}{} & Bit rate    & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\cdot$}                     & {\footnotesize\color{gray50} $\checkmark$}               \\
    \multicolumn{1}{l|}{} & Pragma journal mode                        & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                   \\ 
    \multicolumn{1}{l|}{} & Pragma synchronous          & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}  \\ 
     \multicolumn{1}{l|}{}& Pragma cache size                     & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                    \\ 
    
    \multicolumn{1}{l|}{}  &Pragma page size                       & {\footnotesize\color{gray50} $\cdot$}                                 & {\footnotesize\color{gray50} $\cdot$}    & {\footnotesize\color{gray50} $\cdot$}   & {\footnotesize\color{gray50} $\checkmark$}                     & {\footnotesize\color{gray50} $\cdot$}                  \\ \hlineB{2}  
    \end{tabular}
    }
    {\scriptsize \textsuperscript{\red{a}} Xception+CIFAR10~\cite{chollet2017xception, cifar10} \textsuperscript{\red{b}} BERT+IMDb~\cite{devlin2018bert, maas-EtAl:2011:ACL-HLT2011} \textsuperscript{\red{c}} DeepSpeech~\cite{hannun2014deep}}
    \end{table}
    
